Ties between Parametrically Polymorphic Type Systems and Finite Control Automata

We present a correspondence and bisimulation between variants of parametrically polymorphic type systems and variants of finite control automata, such as FSA, PDA, tree automata and Turing machine. Within this correspondence we show that two recent celebrated results on automatic generation of fluent API are optimal in certain senses, present new results on the studied type systems, formulate open problems, and present potential software engineering applications, other than fluent API generation, which may benefit from judicious use of type theory.

==> baggage.tex <==
the embedding~\cite{Meijer:Beckman:Bierman:06} of \SQL in \CSharp.
\SQL is a domain-specific language for writing database queries.
Consider the \SQL program depicted in \cref{listing:sql:query}.
\begin{JAVA}[language=sql,
  caption={\protect\SQL query},
  label={listing:sql:query}]
SELECT id, name
FROM students
WHERE grade>90
\end{JAVA}
This query is written in native \SQL. A possible method of embedding
the query in an object-oriented programming language is by using an
\SQL fluent API, which may result in the expression shown in \cref{listing:sql:embedded}.
\begin{code}[
  caption={Embedded \protect\SQL query},
  label={listing:sql:embedded}]
Query q=select("id", "name").
          from ("students").
          where (_.grade>90);
\end{code}
The immediate contribution of the fluent API is by providing a \emph{direct
representation} of the original query: All query terminals and literals of
\cref{listing:sql:query} preserve their order on the calls chain of \cref{listing:sql:embedded}.

Alas, it is clear fluent APIs bring additional, possibly unwanted, syntactic
elements; these are usually denoted as \emph{syntactic baggage}, and include:
\begin{description}
  \item[Method call dot (\cc{\underline{.}f})] Method invocations must begin with a dot.
  \item[Method call parenthesis (\cc{f\underline{()}})] Must be present in every
    call, even when lacking arguments.
  \item[Arguments list (\cc{\underline{(}x\underline{,} y\underline{)}})] Literals must come as method call arguments,
    comma-separated.
\end{description}
Instances of syntactic baggage are visible on \cref{listing:sql:embedded}.

Another form of syntactic baggage comes from \emph{naming rules}. Many PLs
forbid some characters from being used in method names: This is an unfortunate pitfall for
fluent APIs, as DSL operators (\cc{+},~\cc{*},~\cc{:}, etc.) cannot be directly
encoded as method names, and therefore should be replaced with strings (\cc{plus},
\cc{by}, \cc{in}, etc.).

The problem of syntactic baggage originates from PLs---but so are the solutions.
\Scala, for instance, is known for being a great host for DSLs†{
\url{https://www.scala-lang.org/old/node/1403}}:
The dot and parenthesis may be omitted from method calls, and method names may
include a wide range of unicode characters, including most operators.

An additional, na\"ive approach is to extend the host language, to contain
the syntax of the DSL. By doing so, language complexity increases with
each DSL added. A more subtle solution has been implemented in the \textsc{.NET}
platform, in the form of \textsc{Linq} \TODO{find citation}:
While query syntax is embedded into the language, query expressions are replaced,
at compile-time, with a chain of fluent API method calls (both look roughly like
\cref{listing:sql:query,listing:sql:embedded}).

\textsc{Linq} demonstrates how fluent API may be used to conceal language extension
in a PL. We observe a more general feature may appease user-defined DSLs, making
syntactic baggage obsolete.

\endinput

It is interesting that previous efforts to introduce XML literals and
expressions into programming languages fail to do the DTD specific type
checking. Such is the case with XJ~\cite{harren2005xj}, an XML extension to
\Java in which all XML instances belong to the same type. Similarly, XML
literals of Visual Basic do not distinguish between various DTDs. Also,
attempts to introduce XML into
\CSharp~\cite{meijer2003unifying,meijer2005xlinq} ignored the issue of static
type checking of distinct XML objects. To our knowledge, the only language
supporting typed XML objects is \textsc{Haskell}~\cite{thiemann2002typed}.
With the current contribution, XML objects with DTD static typing can be easily
introduced into \Java, \CSharp and \CC, for all DTDs that can be written as a
deterministic language. (Note however that a DTD requirement that all rows in
the table have the same number of columns, is not context free, for the same
reason that the language~$aⁿbⁿcⁿ$ is not context free.)


==> completion.tex <==
Suppose that the client of our fluent API library has just typed the partial
call chain \cc{$σ₁$().$⋯$.$σᵢ$()} into the IDE. Then, \emph{auto-completion} by
the IDE means that the client is offered a list of candidates~$ρ₁,…,ρₖ$---the
‟auto-completion list”---to serve in place of~$σ_{i+1}$, the next method in the
chain. Of course, each~$ρⱼ$ should be legitimate, i.e., the IDE should
offer~$ρⱼ$ only if~$σ₁⋯σᵢρⱼ$ can be continued into a word in~$ℓ$, the formal
language of our fluent API.

We draw attention to the fact that a solution for the fluent API problem, does
not necessarily mean an auto-completion feature, and that except for sporadic
comments to say that auto-completion is a desirable feature (e.g.,
in~\cite[page~3]{gil:2016} and in~\cite[page~3]{Nakamaru:17}) the literature largely
ignores the issue of auto-completion. Here we try to fill the gap.

From the theoretical stand point, auto-completion can be thought of
as a generalization of the fluent-API problem.

First, we notice that at least theoretically, auto-completion can be thought of
\begin{property}[auto-completion]\label{property:auto}
  A set of definitions~$D=D(ℓ)$ has the auto-completion
  property if the chain of method calls \cc{$σ₁$().$σ₂$().….$σᵢ$()}
  type-checks against~$D$ if and only if~$∃w∈Σ^*,σ₁σ₂⋯σᵢw∈ℓ$.
\end{property}
\Cref{property:auto} generalizes the fluent API property (\cref{property:fluent})
which constrains~$w=𝜀$. An IDE can utilize the auto-completion property by
adding to the auto-completion list all~$ρⱼ∈Σ$ for which~$σ₁σ₂⋯σᵢρⱼ$
We observe first that a set of definitions~$D(ℓ)$
has the auto-completion property if~$D$ is the fluent API definitions of
the \emph{prefix of}~$ℓ$, defined as \[
  \Prefix(ℓ)=❴w ∣ ∃ w', ww'∈ℓ❵
\] the set of all prefixes of words in~$ℓ$, i.e., all words~$w$ such
that~$ww'∈ℓ$, and that the prefix of a formal language is a special case
of the \emph{quotient of a language~$ℓ₁$ in a language~$ℓ₂$}, defined
as \[
  ℓ₁/ℓ₂=❴w ∣ ∃ w', ww'∈ℓ₁, w'∈ℓ₂❵,
\] i.e., the set of all words that can be completed into a word in~$ℓ₁$ using
only words in~$ℓ₂$. We have~$L/Σ^*=\Prefix(L)$, with~$Σ^*$ a regular language.
Suppose that fluent API definitions are constructed for~$\Prefix(ℓ)$ allows that

by adding a method~$σ∈Σ$ only if
appending it to the call chain does not preclude the possibility that the
call chain is completed to a word in~$ℓ$, i.e., there exists a word~$w'∈Σ^*$
such that~$σ₁⋯σᵢσw'∈ℓ$. When the initial call cannot be completed to a word
in~$ℓ$, i.e., there is no~$w”$ such that~$σ₁,…,σᵢw”∈ℓ$, the auto completion is
ought to be empty, and the IDE should mark the partial chain~$σ₁⋯σᵢ$ as error.

We observe first that, at least theoretically, the problem of auto-completion
is no harder than the fluent API problem:

\begin{corollary}\label{theorem:prefix}
  Suppose that~$ℓ∈C$, where~$ℓ$ is a formal language and~$C$ is a class
  of formal languages, then~$\Prefix(ℓ)∈C$ for~$C$ being the class of
  finite languages, REG, DCFL, CFL and RE.
\end{corollary}
Notice that if~$ℓ$ is context-sensitive, then~$\Prefix(ℓ)$ is in RE†
{\url{https://math.stackexchange.com/questions/3482594/is-language-of-prefixes-of-context-sensitive-language-context-sensitive}}.
\begin{proof}
  Trivial for~$C$ being the class of all finite languages.
  For~$C$ being the class of recursively enumerable languages, simply run
  the Turing machine that enumerates the members of~$L$, modifying
  it so that whenever it enumerates a member of~$L$, it also
  enumerates all prefixes of that member.
  The case of context free languages was settled by Ginsburg~\cite{Ginsburg:1963}
  who showed that the ‟right quotient” of a CFL with a regular language is context-free.
  Ginsburg addressed the deterministic case three years later~\cite{Ginsburg:1966}, yielding
  the corresponding result.
\end{proof}

\subsection{Disposing the error type}

Recall the error type~\cc{ø}, used by Gil and Roth~\cite{gil:2019} to depict
automaton rejection in fluent API. The existence of an error type denies the
auto-completion property; if automaton~$A$ rejects input~$σ₁,…,σₙ,σ_{n+1}$
on~$σ_{n+1}$, then the fluent API of~$A$ might type-check \cc{$σ₁$().….$σₙ$().$σ_{n+1}$()},
yielding~\cc{ø}, instead of raising a compilation error, as required in \cref{property:auto}.
Although not directly addressing this issue, G＆R's work has
been accompanied with a fluent API generator---\Fling, briefly described in
\cite{roth:2019}---composing fluent APIs without the error type.
We now describe \Fling's method of removing~\cc{ø}, and the price
tag that comes along.

Consider class declaration \cc{F<T1,…,Ti,…,Tn>}, taking part in some
fluent API with an error type~\cc{ø}. In a concrete instantiation of~\cc{F},
type variable \cc{Ti} is either~\cc{ø}, or it is not. This bisection can be
expressed in the fluent API, by assuming \cc{Ti} is never~\cc{ø}, and introducing
a new type \cc{F'}, identical to~\cc{F} except \cc{Ti} is fixed to~\cc{ø}.
By using type~\cc{F} one assures \cc{Ti} is not~\cc{ø}, or otherwise backtracks
to \cc{F'} when~\cc{ø} is called upon.

More generally, for each type \cc{F<T1,…,Tn>} introduce~$2ⁿ$ types,
\cc{F$_∅$},…,\cc{F$ₛ$},…,\cc{F$_{❴\text{\cc{T1}},…,\text{\cc{Tn}}❵}$},
where in \cc{F$ₛ$} variable \cc{Ti} is fixed to~\cc{ø} if~$\text{\cc{Ti}}∈s$,
or otherwise it is assumed not to be~\cc{ø}. Assuming a fluent API does not expose
its definitions (i.e., all types are \kk{private}), every occurrence of~\cc{F} can be
replaced with the appropriate \cc{F$ₛ$}, depending on its type arguments. If \cc{Ti}
is~\cc{ø}, then~$\text{\cc{Ti}}∉s$; else, if \cc{Ti} is some type other
than~\cc{ø}, then~$\text{\cc{Ti}}∈s$; otherwise~\cc{F} is being used inside a
class definition \cc{G$ₛ'$<T1',…,Tk'>}, and \cc{Ti} is assigned with some type
variable \cc{Tj'}: in this case \cc{Ti} is~\cc{ø} if~$\text{\cc{Tj'}}∉s'$
(\cc{Tj'}$=$\cc{ø}), or otherwise it remains \cc{Tj'} (\cc{Tj'}$≠$\cc{ø}).

After applying the above transformation, the error type~\cc{ø} can now be safely
removed. Consider return type~$τ$ of some fluent API method: If~$τ$ is some
type variable~\cc{T}, then it is assumed not to be assigned with~\cc{ø}, and remains
untouched; otherwise, if~$τ$ is~\cc{ø}, then the method can be safely removed
(being obsolete), clearing it off the auto-completion lists.

In Gil and Roth's fluent API generation algorithm~\cite{gil:2019}, a type variable
is introduced for every state~$q∈Q$ in the input DPDA; thus, the removal of~\cc{ø}
introduces an \emph{exponential} number of types (in~$|Q|$). Having the original
algorithm producing a fluent API whose size is \emph{polynomial} in the size of
the automaton, the proposed transformation makes the entire ordeal much less appealing.

Fortunately, an obvious optimization can reduce the number of types created.
Under the fluent API scheme, method calls chains start with \kk{static} methods,
i.e., which invoked from no object. For every method, mark each type making an
appearance in its return type as \emph{necessary} for the fluent API; then
repeat the process recursively for every marked type. When finishing, the
types not marked can be safely removed from the fluent API. It remains an
open problem whether this optimization makes the number of types sub-exponential,
considering the fluent API originated from a DPDA, possibly derived from
a context-free grammar, which might influence the final number of types.

\subsection{Translating grammars into early-failure automata}

Gil and Roth's fluent API generator, \Fling~\cite{gil:2019,roth:2019},
accepts a deterministic context-free grammar as input, converts
it into a DPDA, and then composes the automaton as a fluent API.
As it appears, accepting grammar as input---rather
than a raw automaton---is not only comfortable, but also makes
it possible to create auto-completion-aware fluent APIs.

First, we define the \emph{early-failure} property of automata, similar
to \cref{property:auto} of fluent APIs:
\begin{property}[early-failure]\label{property:failure}
  Let~$A$ be an on-line†{accepting input letter-by-letter} automaton
  accepting language~$ℓ$.
  Automaton~$A$ \emph{hangs} after consuming input word~$w$, if and only if
  $\not ∃ w',\ ww'∈ℓ$.
\end{property}
An early-failure automaton rejects its input as soon as it cannot be completed
to an accepted word.
Works that encode an automaton in the type-system as a fluent
API~\cite{gil:2016,Grigore:2017,Nakamaru:17,gil:2019} have the fluent API fail
compilation on automaton rejection:
So by supplying their algorithms with early-failure automata,
we get fluent APIs holding the auto-completion property.

Our goal is to…Assume language~$ℓ$ is described by an automaton~$A$:
then a common blunder is to allow a chain~$w$ to compile as long as~$A$
does not get stuck, even if~$w$
is not a prefix of an~$ℓ$ word. Gil and Levy~\cite{gil:2016} and Gil and
Roth~\cite{gil:2019} go even further to introduce an \emph{error type}~\cc{ø}, to
be returned from aborted chain; Having a method return~\cc{ø} implies
not only it can be called without raising a compilation error, but also
that it appears on the auto-completion list.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lemma:ll1:dpda}
  Let~$G$ be an~$LL(1)$ grammar of language~$ℓ$.
  We may construct a DPDA~$A$ accepting~$ℓ$, where the stack of
  $A$ is equal to the stack of~$G$ during parsing.
\end{lemma}
\begin{proof}
  Introduce state~$q₀$. Computation starts in state~$q₀$, and after
  consuming an input letter, it would end in~$q₀$.
  Introduce state~$q_σ$ for every terminal~$σ$ in~$G$:
  When letter~$σ$ is read, move to~$q_σ$; an~$LL(1)$ derivation
  rule can be carried out by the DPDA, by simply reading the variable from
  the stack's top, and replacing it with the right-hand side of the
  appropriate rule, considering~$σ$. When~$σ$ is derived, then
  move to~$q₀$.

  The DPDA should accept the input after consuming a letter if all the
  variables in its stack may be derived to~$𝜀$. To do this,
  introduce state~$q₀^\$$ and a symbol~$V^\$$ for every grammar variable
  $V$. If variable~$V₁$ is to be pushed onto~$V₂^\$$, and~$V$ can be derived
  to~$𝜀$, then push~$V₁^\$$; otherwise if~$V₁$ if not nullable,
  or is pushed onto~$V₂$, then push~$V₁$ instead. Finally, make~$q₀^\$$
  accepting, and move from~$q₀$ to~$q₀^\$$ if the top symbol is annotated
  with~$\$$, and vise versa.
\end{proof}

\begin{theorem}
  Let~$G$ be an~$LL(1)$ grammar of language~$ℓ$.
  An early-failure DPDA accepting~$ℓ$ can be constructed from~$G$.
\end{theorem}
\begin{proof}
  Consider DPDA~$A$ accepting~$ℓ$, constructed from~$G$ in \cref{lemma:ll1:dpda}.
  Having no left-recursion in~$LL(1)$ grammars means a computation in~$A$
  always halts. To have early-failure,~$A$ should immediately reject the input
  when~$σ$ has been read, and it cannot be derived; this can be achieved
  by completely emptying the stack, when variable~$V$ (or~$V^\$$) is at the
  stack's top in state~$q_σ$, and~$σ∉\text{\sffamily firsts}(V)$†{
  The set~$\text{\sffamily firsts}(V)$ contains all terminals that can be derived as
  the first symbol of~$V$.}.
\end{proof}


==> deadwood.tex <==
Notice pushdown automata are also tree automata, whose tree memories are linear.
Considering \cref{lemma:ta:rt}, we get that any DCFL can be accepted in real
time by a tree automaton, \[
  \PP=\text{TA}\supseteq \text{DPDA}.
\] This result is the same as that of \GR, preceding it by 36 years†{Gil and
Roth's construction, though, is straight-forward, in contrast to Guessarian's,
which requires a translation of the tree automaton to a tree grammar, a grammar
transformation and then a translation back to tree automaton.}.

The \emph{restricted PDTA} (RPDTA) of
Guessarian~\citeyear{Guessarian:83} fixes the storage tree to be
linear; having the input linear as well, an RPDTA is exactly a PDA.

\begin{lemma}[\normalfont Theorem 3 of~\cite{Guessarian:83}]\label{lemma:ta:pda}
  Any language accepted by a PDTA can be accepted by a restricted PDTA.
\end{lemma}

Observe Guessarian's proof of the corresponding theorem preserves
determinism†{We have worked out a proof of our own, but it is very similar to
  Guessarian's, so it was removed;
we are convinced modifying the construction of Guessarian to fit the
deterministic case is a matter of technical work.}, i.e., a shallow,
(non-)real-time tree automaton can be converted to a DPDA, therefore \[
  \PP=\A[TA]{$𝜀$-transitions}⊆\text{DPDA}.
\] (The first equivalence is by \cref{lemma:ta:rt}.)
Following \cref{lemma:ta:pda}, it is possible to type check \PP programs using
a DPDA: Given a program, we convert it into a tree automaton, and use the construction of
\cref{lemma:ta:pda} to produce a DPDA~$A$. Then, to type check an expression is
simply to run it on~$A$.

\begin{proof}[Proof of \cref{theorem:pp:dcfl}]
  Derived from \cref{lemma:ta:rt,lemma:ta:pda}, as explained above.
\end{proof}


Consider \PP with deep patterns, \A[\PP]{deep}, where function may have deep
argument types, e.g.,~$σ:γ(γ(γ(X)))→τ$. Adding deep types to \PP make it
stronger---a potent result, considering many real world type systems are
classified by \A[\PP]{deep}, i.e., parametric polymorphism without fluent APIs.
Consider the \A[\PP]{deep} reverse fluent API of \cref{listing:sd:anbncn},
accepting the language~$ℓ=aⁿbⁿcⁿ$, known to be context sensitive.

\begin{lemma}\label{lemma:ta:rt}
  RDPDA=DPDTA is equivalent to a real-time DPDTA.
\end{lemma}

\begin{proof}
[\normalfont Corollary 1.\1 of~\cite{Guessarian:83}]
\end{proof}
Using our terminology, Guessarian showed any \A[TA]{$𝜀$-transitions} automaton
can be converted into an equivalent tree automaton, which has no~$𝜀$-transitions,
and which employs a single state. (Guessarian's construction uses a single
state.)
\subsection{Background}
This paper is concerned with \emph{compile time computation}, specifically
computation which is carried out by the type checker: From the theoretical
perspective, compile time computation is the reduction of an instance of
decision problems, or equivalently, membership in some class of formal
languages, to an instance of a type checking in a given type system.

The main practical motivation of compile time computation is the rising
interest in automatic synthesis of fluent API libraries (see Yamazaki et
al.~\cite{Yamazaki:2019} for a recent survey). As observed
previously~\cite{gil:2016}, this synthesis boils down to the problem of
coercing the type checker to do the task of recognizing a formal language.

Compile time computation is particularly intriguing in \emph{decidable} type
systems. This is because Turing complete type systems are not fun adverse effects on
usability of the programming language~\cite{}. Secondly, the question of
compile time
computation loses its challenge in such systems. For these reasons our work
also highlights components of the type system which render it Turing complete.

We present a \emph{taxonomy} (see \cref{figure:taxonomy} below) of parametrically
polymorphic type systems
with parametric polymorphism and the \emph{correspondence} between these
systems and formal languages, or,
almost equivalently, to models of computation, starting at finite state machine
going through, e.g., linear bounded automaton, and ending with a Turing
machine.

In this taxonomy we show e.g., that the celebrated encoding of fluent APIs
whose underlying language is LR, i.e., language admitting left to right
parsing, in a no-variance polymorphic type system~\cite{gil:2016,gil:2019} is
the best possible: i.e., if this type system recognizes a certain language,
this language must be LR. This lower bound result is obtained from the
observation that polymorphic type systems are best described by \emph{auxiliary
tree automata}; the same observation leads to a much simpler representation of
the said encoding.

Some of the type system varieties we identify are not bound as tightly, i.e.,
there is gap between what we know that can be computed by the type system, and
what we know that cannot be computed on it. Filling each of these gaps may be
an interesting future research.

We notice that a Java back-end for \TypelevelLR is theoretically possible, but
completely impractical.


==> definitions.tex <==
\subsection{Definitions}
To make the material in \cref{section:automata} more accessible, here we
repeat, expand, and exemplify the definitions of trees, terms, substitutions
and rewrites.

Alphabet~$Γ$ is a \emph{signature} if each~$γ∈Γ$ has a positive integer
\emph{rank}. Let~$Γᵣ$ be the set of those elements of~$Γ$ whose rank is~$r$.
Let~$𝜀∉Γ$ denote the \emph{universal leaf}. Then,~$Γ^▵$ is the set of all
\emph{ground terms} (also called \emph{trees})
over~$Γ$, i.e., finite structures of the form~$γ(t₁,…,tᵣ)$, where~$γ∈Γᵣ$,
and where every~$tᵢ$,~$i=1,…,r$, is either~$𝜀$ or a grounded term itself,
i.,e.,~$tᵢ∈Γ^▵$. Note that if~$Γᵣ=∅$ for~$r≥2$, then~$Γ^▵$ is
(essentially)~$Γ^*$.  We use \emph{monadic tree abbreviation} by which
tree~$γ₂(γ₁(𝜀),γ₁(γ₁(𝜀)))$ is written as~$γ₂(γ₁,γ₁γ₁)$, and
tree~$γ₁(γ₂(⋯(γₙ(𝜀))))$ is written as~$γ₁γ₂⋯γₙ$.


We use signature~$❴γ₁,γ₂,γ₃❵$, with~$γᵢ$ having rank~$i$,~$i=0,1,2,3$ in our
examples. \Cref{figure:trees} depicts a definition of example terms~$t₀,…,t₆$
in this signature.

\begin{figure}[ht]
  \caption{Definition of grounded terms~$t₀,…,t₆∈❴γ₁,γ₂,γ₃❵^▵$.}
  \label{figure:trees}
  \adjustbox{max width=\textwidth}
  {\input{trees.tikz}}
\end{figure}

We also use the notion of \emph{sub-tree}, e.g., in the figure,~$t₂$ is a
sub-tree of~$t₅$ and~$t₃$ is a sub-tree of~$t₆$. Every tree is a sub-tree of
itself. The depth of a tree is defined as usual, e.g., the depth of~$t₀$ is~0,
the depth of~$t₁$,~$t₂$ and~$t₃$ is~1, and the depth of~$t₄$,~$t₅$ and~$t₆$
is~2.

Let~$X=❴x₁,x₂,…❵$ be an infinite set of \emph{(formal) variables}, disjoint to
any alphabet. Let~$Γ⧋$ be the set of \emph{terms} over~$Γ$, comprising trees
whose internal symbols are drawn from~$Γ$ and leaves are drawn from~$Γ∪X$.
Stated differently,~$Γ⧋$ is the smallest superset of~$X$ that
contains~$γ(τ₁,…,τᵣ)$ whenever it contains~$τ₁,…,τᵣ$ and~$γ∈Γᵣ$.

\Cref{figure:terms} depicts the definition of example terms~$τ₀,…,τ₆$ in this signature.

\begin{figure}[ht]
  \caption{Definitions of terms~$τ₀,…,τ₆∈❴γ₁,γ₂,γ₃❵⧋$.}
  \label{figure:terms}
  \adjustbox{max width=\textwidth}
  {\input{terms.tikz}}
\end{figure}

For~$τ∈Γ⧋$ let~$\Vars(τ)⊂ X^*$ be the multi-set of formal variables occurring
in~$τ$, e.g.,~$\Vars(τ₃)=❴x₁,x₂,x₃❵$ and~$\Vars(τ₄)=❴x₁,x₁,x₂❵$. Term~$τ$ is
\emph{linear} if~$\Vars(τ)$ is a set, i.e., no variable occurs in~$τ$ more than
once. The only non-linear term in \cref{figure:terms} is~$τ₄$.

Every grounded term~$t$ is also a term with~$\Vars(t)=∅$, so~$Γ^▵⊊Γ⧋$.

A \emph{substitution} is a set of \emph{substitution
rules}~$s=❴x₁↦τ₁,…,xₙ↦τₙ❵$, where~$x₁,…,xₙ∈X$ are distinct variables
and~$τᵢ∈Γ⧋$. Let~$τ/s$, the \emph{application} of~$s$ to~$τ$, be the term
obtained from~$τ$ by replacing each leaf of it labeled~$xᵢ$ with the term~$τᵢ$.
For example, \[
  \begin{split}
    τ₃/❴x₁↦x₂,x₂↦γ₁(x₁),x₃↦𝜀❵&=γ₃(x₁,x₂,x₃)/❴x₁↦x₂,x₂↦γ₁(x₁),x₃↦𝜀❵ ⏎
    &=γ₃(x₂,γ₁(x₁),𝜀) ⏎
    &=τ₅.
  \end{split}
\] A \emph{grounded} substitution is a substitution in which$τ₁,…,τₙ$ are
grounded, e.g.,~$❴x₁↦𝜀,x₂↦γ₁,x₃↦𝜀❵$ is grounded and \[
  τ₃/❴x₁↦𝜀,x₂↦γ₁,x₃↦𝜀❵=γ₃(x₁,x₂,x₃)/❴x₁↦𝜀,x₂↦γ₁,x₃↦𝜀❵=t₄.
\] A \emph{renaming} is a substitution in which~$τ₁,…,τₙ∈X$,
e.g.,~$❴x₁↦x₂,x₂↦x₁❵$ is a renaming, and \[
  γ₂(x₁,x₂)/❴x₁↦x₂,x₂↦x₁❵=γ₂(x₂,x₁).
\] We think of term~$τ$ as \emph{pattern} over trees, and more generally, over
terms: If there is substitution~$s$ such that~$τ'=τ/s$, then we write~$τ'⊑τ$
and say that~$τ'$ is \emph{matched} by~$τ$. If~$τ'$ has a sub-tree~$τ”⊑τ$, then
we say that~$τ'$ \emph{matched by~$τ$ \underline{at}~$τ”$}.

For example,~$t₅$ is matched by~$τ₄$ with substitution~$❴x₁↦𝜀,x₂↦𝜀❵$.
Also,~$t₆$ matches pattern~$τ₃$ both \underline{at}~$t₆$ itself with
substitution~$❴x₁↦𝜀,x₂↦𝜀,x₃↦γ(𝜀,𝜀,𝜀)❵$, and \underline{at}~$t₃$ with
substitution~$❴x₁↦𝜀,x₂↦𝜀,x₃↦𝜀❵$.

It is easy to verify that if~$τ$ matches~$t$ at~$t'$, then~$t$,~$t'$ and~$τ$
determines the substitution~$s$ (up to renaming and immaterial or redundant rules)
and that~$s$ must be grounded.

If~$τ,τ'∈Γ⧋$ are terms such that~$\Vars(τ')⊆\Vars(τ)$, the notation~$τ→τ'$ stands
for a \emph{rewrite rule}. For example, \Cref{figure:rules} defines rewrite
rules~$ρ₁,ρ₂,ρ₃,ρ₄,ρ₅,ρ₆,ρ₇$ on the signature~$❴γ₁,γ₂,γ₃❵$.

\begin{figure}[ht]
  \caption{A rewrite system~$❴ρ₁,ρ₂,ρ₃,ρ₄,ρ₅,ρ₆,ρ₇❵$ over
    signature~$❴γ₁,γ₂,γ₃❵$.}
  \label{figure:rules}
  \adjustbox{max width=\textwidth}
  {\input{rules.tikz}}
\end{figure}

A \emph{rewrite} of grounded term~$t$ by rule~$τ→τ'$ requires a match of~$τ$
at~$t'$ with substitution~$s$. In the rewrite a sub-tree~$t'$ of~$t$ is replaced
by~$τ'/s$. A rewrite is \emph{shallow} if~$t'=t$ (and therefore~$t⊑τ$); it is
\emph{deep} if~$t'$ is a proper sub-tree of~$t$. Let~$ρ(t)$ denote the tree
obtained by applying rule~$ρ=τ→τ'$ in a shallow rewrite to tree~$t$;~$ρ(t)$ is
undefined if~$τ$ does not match~$t$.

We are safe to assume that rules are written in \emph{canonical form} in which
variables occur in the left occur in ascending numerical order~$x₁,x₂,…$. All
rules in the figure are in canonical form. A stray rule such
as~$γ₂(x₅,γ₂(x₄,x₅))→γ₂(x₄,x₅)$ can be always rewritten in canonical form by a
renaming that preserves its semantics,~${x₅↦x₁,x₄↦x₂}$ for rule in point.

Consider, for example, the application of rule~$ρ₄$ to tree~$t₆$: The match of
pattern~$τ₃$ at the left hand side of the rule with~$t₆$ at~$t₃$ rewrites~$t₆$
to~$γ₃(𝜀,𝜀,t₅)$; the match of this pattern with the rewritten~$t₆$ at its
root rewrites it to~$t₅$.

A rewriting rule~$τ→τ'$ is \emph{extracting} if~$τ'∈X$, and~$τ∉X$, i.e., the
rule rewrites a term into a variable that occurs in this term; otherwise it is
\emph{accumulating}. In~\cref{figure:rules} only rules~$ρ₁$ and~$ρ₂$ are
extracting, and the others are accumulating. Degenerate rules such
as~$γ₂(x₁,x₂)→γ0$,~$x₁→𝜀$, and~$x₁→γ₁$ in which the rule's right does not
contain a variable are considered accumulating and so is the no-op rule~$x→x$.

A rewrite system is~$R$ is a set of rewrite rules;~$R$ is \emph{linear} if
terms in the left of its rules are linear, i.e., for every rule~$τ→τ'∈R$,
term~$τ$ is linear. Thus, the rewrite system in \cref{figure:rules} is
linear, even though some terms in the right hand of its rules are not linear.
The \emph{depth} of a rewrite system is the maximal depth of terms on the left
of rules. The depth of the system in the figure is 1.

\subsection{Alternative Proof of \cref{lower:bound}}
\label{section:lower:bound}
A monadic TPDA receives as input a tree of degenerate form---a chain, and
processes this chain bottom up, using a single tree drawn from~$Γ^▵$ as
auxiliary storage. Thus, a monadic TPDA is similar to a PDA except that the
auxiliary storage a PDA may use is restricted to be a stack. In this section,
we show that this restriction does not reduce the expressive power of an
automaton: Monadic TPDAs are not more powerful than PDAs.

\begin{theorem}\label{theorem:monadic}
  Any language recognized by a monadic TPDA is also recognizable by PDA.
\end{theorem}
The proof is by construction: Given a monadic TPDA~$T$, we describe a PDA~$A$
that emulates~$T$: every run of~$T$ on a given input, has an equivalent run
of~$A$ on the same input, such that the run on~$T$ is accepting if and only if
the run on~$A$ is accepting. Let~$T=⟨Σ,Q,Γ,F,R⟩$, and suppose that the rank
of~$Γ$ is~$m$. Then, we construct~$A=⟨Σ,Q',q₀,F,Γ',⊥,δ⟩$ as follows:
\begin{enumerate}
  \item By writing the monadic input tree~$σₙ(σ_{n-1}(⋯(σ₂(σ₁()))⋯))∈Σ^▵$ as the
        string~$σ₁σ₂⋯σₙ∈Σ^*$, we can let~$A$ use the same input alphabet as~$T$.
  \item Also,~$A$ relies on the same set of states as~$T$, except that we introduce
        an initial state~$q₀∉Q$ for~$A$, and allow~$A$ to use intermediate states
        drawn from~$Q×❴1,…,k❵$ during the emulation, i.e.,~$A$'s states are
        states \[
          Q'=❴q₀❵∪Q∪Q×❴1,…,k❵.
\] However, the set~$F$ of final states is the
        same in~$T$ and in~$A$.
  \item Similarly introduce a new bottom of stack symbol~$⊥∉Γ$.
        Other stack symbols in~$Γ'$, the set of stack symbols of~$A$,
        are constructed from the rewrite rules~$R$ as explained
        below with the description of the transition function~$δ$.
\end{enumerate}

\subsection{Intuition}
\label{section:intuition}

First notice that we can assume that standard rules in~$R$ are in the special
form~$σ(q(τ))→q(τ)$, by which the input letter is consumed, a state transition
is made, but the tree over~$Γ$ does not change. The assumption is made possible
by converting standard rule~$σ(q(τ))→q'(τ)$ to two rules:
\begin{enumerate}
  \item standard rule~$σ(q(τ))→q_{σ,τ}(τ)$ to consume input letter~$σ$ and to
        record the remaining transformation of the current tree in a newly
        introduced state~$q_{σ,τ}$ of automaton~$T$, and
  \item reduce rule~$q_{σ,τ}(τ)→q'(τ')$ to carry out this remaining transformation
        from~$τ$ to~$τ'$.
\end{enumerate}

Examine the four possible forms that may be taken by a rewrite rule of a monadic TPDA:
\begin{equation}\label{eq:transitions}
  \begin{array}{lr}
    σ(q(τ))→q'(τ) & \text{\qquad\slshape standard rule, inner node}. ⏎
    σ()→q(τ) & \text{\qquad\slshape standard rule, leaf node}. ⏎
    q(x)→q'(τ') & \text{\qquad\slshape reduce rule, any node,~$x∈X$} ⏎
    q(γ(x₁,…,xₖ))→q'(τ') & \text{\qquad\slshape reduce rule, compound node,~$x₁,…,xₖ∈X$} ⏎
  \end{array}
\end{equation}
We see that tree rewrites by these rules can be decomposed to two orthogonal
changes to the instantaneous description of~$A$:
\begin{enumerate}
  \item A state transition from~$q$ to~$q'$, possibly consuming input letter~$σ$, and
  \item a shallow rewrite of the current tree in~$Γ^▵$, by rules of either
        the form~$x→τ'$ or the form~$γ(x₁,…,xₖ)→τ'$, where~$x₁,…,xₖ∈X$.
\end{enumerate}
The first kind of changes are readily emulated by a PDA whose management of the
current input letter and the changes of state are similar to that of a
monadic TPDA; indeed, the finite control of the two kinds of automata are equivalent.
The challenge of the emulation is in using the PDA's stack to encode the
grounded term over~$Γ$ that the TPDA currently manipulates.

To see that a plain prefix order encoding of a tree in a stack does not work,
consider applying the reducing rewrite rule~$ρ₆=γ₂(x₁,x₂)→γ₃(x₂,γ₁(x₁),γ₀)$ to
tree~$γ₂(t₁,t₂)$,~$t₁,t₂∈Γ^▵$. In prefix order the stack is~$γ₂α₁α₂⊥$
where~$αᵢ$ is the stack encoding of tree~$tᵢ$,~$i=1,2$. To emulate the rewrite
a PDA moves to state~$q'$ and pops~$γ₂$. But then, to maintain prefix encoding
the remaining stack~$α₁α₂⊥$ should be rearranged to~$γ₃α₂γ₁α₁γ₀⊥$. Alas, the
unbounded length of~$α₁$ and~$α₂$ makes this rearrangement impossible in the
bounded memory available to a PDA other than the stack itself.

A better encoding of the TPDA's tree by letting the PDA's stack employ rewrite
rules as its symbols: a tree~$t∈Γ^▵$ is encoded as a sequence of applications
of \emph{accumulating} rewrite rules stored in a stack, with the latest rewrite
at the stack's top. The earliest rewrite, stored at the stack's bottom is rule
of the form~$⊥→t$,~$t$ being a grounded term over~$Γ$, e.g., an encoding of the
leaf node~$γ₀$ is the sequence comprising the single rule~$ρ₀=⊥→γ₀$.
Also,~$ρ₃ρ₅ρ₀⊥$ is a stack encoding of~$t₅=γ₂(γ₂(γ₀,γ₀),γ₀)$, since applying
rule~$ρ₅$ to~$γ₀$, and then~$ρ₃$ yields~$t₅$. The encoding is not unique, e.g., \[
  \overbrace{ρ₃⋯ρ₃}ⁿρ₅γ₀⊥
\] is a stack encoding of~$t₅$ for all odd values of~$n$.

With this encoding, an application of any accumulating rewrite rule~$ρ$ to the
current tree is emulated by pushing~$ρ$ onto the stack. For example,
applying~$ρ₆$ and then~$ρ₄$ to tree~$t₅$ yields the
term~$γ₂(γ₂(γ₁(γ₀),t₂),t₂)$; to encode this term, rules~$ρ₆$ and~$ρ₄$ are
pushed onto the stack, as depicted in~\cref{figure:stack}.

\begin{figure}[H]
  \caption{Stack contents
    after applying rewrite rule~$ρ₅$, then~$n$ times~$ρ₃$ for some
    odd~$n$, then~$ρ₆$, and finally~$ρ₄$ to~$ρ₀=⊥→γ₀$.}
  \label{figure:stack}
  \adjustbox{max width=\textwidth}
  {\input{stack.tikz}}
\end{figure}

%To see that the encoding makes it is possible to match rules against the
%current tree in its encoded form, we assume for now that rewrite rules of the
%form~$γ(v₁,…,vₖ)→τ$ are restricted to the form~$γ(x₁,…,xₖ)→τ$, i.e., there are
%no rules such as~$γ₂(γ₃(⋯),x₁)→τ$ in which one alphabet symbol ($γ₃$) occurs as
%argument of another alphabet symbol~($γ₂$) in the left hand size of the rule.
%Later we will see how this assumption can be lifted.
%With this assumption and the presumed linearity of rules.

The PDA's finite control can use the stack's top to decide whether a certain
rule is applicable to the current tree. Rule~$ρ₄$ at the top of the stack in
the figure confirms that the current tree is of the form~$γ₂(t₁,t₂)$
with~$t₁,t₂∈Γ^▵$. Rules~$ρ₁$,~$ρ₂$,~$ρ₃$ and~$ρ₆$, indeed all rules whose left
hand is the term~$γ₂(x₁,x₂)$, match this tree. Regardless of the stack's top,
the current tree is matched by~$ρ₇$, and, more generally all rules of the
form~$x→τ$ whose left does not place any constraints on the matched tree.

As said, the encoding is preserved by always pushing accumulating rules.
Managing extracting rules is more tricky, requiring sometimes an unbounded
sequence of pop operations: Consider the application of extracting
rule \[
  ρ₂=γ₂(x₁,x₂)→x₂
\] to the stack depicted in \cref{figure:stack}. To
extract the \emph{second} child of the current tree we inspect rule~$ρ₄$ at the
top of the stack to infer that this second child is variable~$x₁$ of the
term~$γ₃(x₁,x₂,x₃)$ that matched the current tree prior to the application
of~$ρ₄$. Popping~$ρ₄$ obtains the stack encoding of the previous version of the
current tree. On this shorter stack, we need to find the first child
of~$γ₃(x₁,x₂,x₃)$. Popping rule~$ρ₆$, the problem is reduced to finding second
child of a tree~$γ₂(x₁,x₂)$. To encode the current tree after the rewrite~$ρ₂$
we need to further pop the~$n$ copies of~$ρ₃$ and then replace rule~$ρ₅$ at the
top of the remaining stack with rule~$γ₀→γ₂(γ₀,γ₀)$.

A similar replacement of the rule at the stack's top occurs when applying
rule~$ρ₁=γ₂(x₁,x₂)→x₁$ that extracts the first child of the tree encoded in the
figure. The right of~$ρ₄$, term~$γ₂(γ₂(x₂,x₁),x₁)$, specifies how this first
child depends on the tree before applying~$ρ₄$. Accumulating
rule~$ρ₄'=γ₃(x₁,x₂,x₃)→γ₂(x₂,x₁)$ then describes the combined application
of~$ρ₄$ and~$ρ₂$, and the encoding is preserved by replacing~$ρ₄$ by~$ρ₄'$ at
the top of the stack.

\subsection{The Transition Function}
Having gained the intuition of the emulation, we now turn to providing the
technical details of the emulation behind the proof
of~\cref{theorem:monadic}.

Recall that PDA~$A$ uses the same alphabet as~$T$, and its set of states
is~$Q'=❴q₀❵∪Q∪Q×❴1,…,k❵$. The set~$Γ'$ of stack symbols of~$A$ comprises the
special bottom of stack symbol~$⊥$ and rules of the form~$τ→τ'$,
where~$τ∈❴⊥❵∪Γ⧋$ and~$τ'∈Γ⧋$.
It remains to describe~$δ$, the transition function of~$A$.

We say that an accumulating rewrite rule~$ρ'∈Γ'$ \emph{follows} another
accumulating rewrite rule~$ρ∈Γ'$ and write~$ρ⤳ρ'$, if~$ρ'$ is applicable after
applying~$ρ$. More exactly,~$ρ⤳ρ'$ if~$ρ'$ is a shallow match of every
tree encoded by a stack of the form~$ρα⊥$, for arbitrary~$α∈(Γ')^*$.

Considering the rules in \cref{figure:rules} we see that rule~$ρ₆$ which
assumes a tree whose root is~$γ₂$ follows~$ρ₃$,~$ρ₄$ and~$ρ₅$. Also, yields a
tree with root~$γ₃$, rule~$ρ₆$ is followed by~$ρ₄$ which requires~$γ₂$ root of
the input tree, and by rule~$ρ₇$ which is applicable to any tree.

%More
%generally, with the assumption an alphabet symbol cannot occur as an
%argument of another alphabet symbol in the left hand size of the rule, we can
%tell whether~$ρ⤳ρ'$ solely by comparing the root of the term in the right~$ρ$
%with the root of the term in the left of~$ρ'$.

More generally, with the restriction that at most one stack
node occurs in the left hand size of the rule, we can
tell whether~$ρ⤳ρ'$ solely by comparing the root of the term in the right~$ρ$
with the root of the term in the left of~$ρ'$.

For each rewrite rule present in~$R$, we construct transition(s) as follows.
Even with our simplifying assumption on the structure of standard rules,
There are quite a number of cases to consider:
\begin{description}
  \item[Standard Rules] By our transformation, these rules do not manipulate the tree storage.
        They come in two varieties:
        \begin{enumerate}
          \item~$σ(q(τ))→q'(τ)$, \emph{standard rule, inner node}: Introduce a
                transition~$(q,σ,ρ)→(q',ρ)$ for every stack symbol~$ρ$. These
                transition preserve the stack, consume letter~$σ$ and move to state~$q'$.
          \item~$σ→q(t)$, \emph{standard rule, leaf node}: Introduce stack
                symbol~$ρ=⊥→t$ and transition~${(q₀,σ,⊥)→(q,ρ⊥)}$. This transition
                initializes the stack with a rewrite that generates a non-empty tree~$t∈Γ^▵$
                from the stack's bottom.
        \end{enumerate}
  \item[Reduce Rules] Such a rule does not consider the input. It can be
        accumulating, and hence emulated by being pushing onto the stack,
        or extracting, and then emulated by a sequence of an unbounded number of
        stack pop operations, followed by a push of a new rule:
        \begin{enumerate}
          \item~$q(τ)→q'(τ')$, \emph{accumulating reduce rule}: Introduce stack
                symbol~$ρ'=τ→τ'$ and create transition~$(q,𝜀,ρ)→(q',ρ'ρ)$ for
                every~$ρ∈Γ'$ that satisfies~$ρ⤳ρ'$, i.e., push~$ρ'$, move
                to state~$q'$. This rule is applicable if the current state is~$q$
                and the stack's top, rewrite rule~$ρ$ is such that~$ρ'$ is
                applicable to the tree encoded in the stack.

          \item~$q(x)→q'(x)$, \emph{degenerate accumulating reduce rule}:
                Create transition~$(q,𝜀,ρ)→(q',ρ)$ for every~$ρ∈Γ'$. These
                transitions leaves the stack intact, but move from state~$q$ to
                state~$q'$.

          \item~$q(γ(x₁,…,xₖ,…,xᵤ))→q'(xₖ)$, \emph{extracting reduce rule},
                where~$u≤m$ is the rank of symbol~$γ$, and~$k$,~$1≤k≤u$, is the
                index of the extracted variable. Let the stack's top be
                rule~$ρ=τ→τ'$. We must then create transitions to extract~$τ'[k]$,
                the~$k$\xth child of~$τ'$, while preserving the stack encoding.

                \begin{enumerate}
                  \item If~$τ'[k]$ is a term which is not a variable, then as done
                        above in the application of~$ρ₁$ after~$ρ₄$, introduce a stack
                        symbol~$ρ'=τ→τ'[k]$. Rule~$ρ'$ is similar to~$ρ$, but rather
                        than rewriting the encoded tree to the full term~$τ'$, it
                        rewrites it to its subtree~$τ'[k]$. Rule~$ρ'$ is accumulating
                        by the assumption~$τ'[k]∉X$, and can therefore be used as a
                        symbol in the stack encoding of trees. To replace~$ρ$ by~$ρ'$
                        at the top of the stack, introduce
                        transition~$(q,𝜀,ρ)→(q',ρ')$. This transition also moves from
                        state~$q$ to state~$q'$.

                  \item Suppose that~$τ'[k]∈X$. Since~$ρ=τ→τ'$ is a
                        rule,~$\Vars(τ')⊆\Vars(τ)$, variable~$τ'[k]∈X$ must be present
                        in~$τ$. By the restrictions on monadic~$T$,~$τ$
                        is either a variable or a compound term of the form~$γ'(x₁,…,x_{u'})$.

                        If~$τ$ is also a variable, then it must be the variable~$τ'[k]$,
                        so~$τ'[k]$ is precisely the tree encoded by the stack prior to
                        the application of~$ρ$. Introduce then
                        transition~${(q,𝜀,ρ)→(q',𝜀)}$, which pops~$ρ$ from the stack
                        and moves to~$q'$.

                        Otherwise,~$τ'[k]$ is variable~$xᵢ$ appearing in~$τ=γ'(x₁,…,x_{u'})$.
                        Automaton~$A$ must proceed to extract the~$i$\xth child of the
                        tree prior to the rewrite~$ρ$. Introduce then
                        transition~${(q,𝜀,ρ)→(⟨q',i⟩,ρ)}$, which leaves the stack
                        intact, but moves to intermediate state~$⟨q',i⟩$. Being in
                        state~$⟨q',i⟩$ tells~$A$ to ‟\emph{extract child~$i$ of the
                          currently encoded tree and then move to state~$q'$}”.
                \end{enumerate} % inner
        \end{enumerate} % outer
\end{description}

We still need to add transitions to realize the intent of the above mentioned
intermediate states. For intermediate state~$⟨q,k⟩$ and rule~$ρ=τ→τ'$, where
the rank of the symbol in the root of~$τ'$ is no less than~$k$, let~$τ'[k]$ be
the~$k$\xth child of~$τ'$, and,
\begin{itemize}
  \item if~$τ'[k]∉X$, introduce accumulating rule~$p'=τ→τ'[k]$ as stack symbol, and
        transition~$(⟨q,k⟩,𝜀,ρ)→(q,ρ')$ to move to destination state~$q$ and
        replace a top of stack~$ρ$ with~$ρ'$ whenever in state~$⟨q,k⟩$ and top
        of stack is~$ρ$;
  \item if~$τ'[k]$ is a variable~$x$ then~$τ=x$. Introduce then
        transition~$(⟨q,k⟩,𝜀,ρ)→(q,𝜀)$ to pop~$ρ$ and move to destination state~$q$.
  \item otherwise,~$τ'[k]$ is some variable~$xᵢ$;
        then introduce transition~$(⟨q,k⟩,𝜀,ρ)→(⟨q,i⟩,𝜀)$ to pop~$ρ$ and
        proceed the search down the stack for the~$i$\xth child of the tree encoded
        by the remaining stack, and then move to state~$q$.
\end{itemize}

We therefore have that accumulating rules of~$R$ are emulated by precisely one
transition from state~$q$,~$q∈❴q₀❵∪Q$ to state~$q'∈Q$. Extracting rules
of~$T$ are emulated by an unbounded number of transitions, starting in~$q∈Q$,
possibly going through some intermediate states of the form~$⟨q',·⟩$, each
popping a rule of the stack, and ending in a state~$q'∈Q$ and a push of a rule.

Review the definition of~$δ$ to better understand the set~$Γ'$: A standard
rule in~$R$ that operates on a leaf node introduced a symbol of the form~$⊥→t$.
A reduce rule in~$R$ could be accumulating, in which case it introduces a
single element to~$Γ'$. However if this rule is extracting,
it can introduce many. Observe however that a rule~$p'$ is introduced only if
there exists a rule~$ρ∈Γ'$ such that~$ρ=τ→τ'$ and~$ρ'=τ→τ'[k]$. Since the
description of~$ρ'$ is shorter than the description of~$ρ'$, set~$Γ'$ must be
finite.

% Although not strictly necessary for the proof of \cref{theorem:monadic}, we
% explain now how the emulation is extended to handle rules such
% as~$γ₂(γ₃(⋯),x₁)→τ$: To make this happen, we need to extend the~$⤳$ relation
% so that it supports matches of patterns~$γ(v₁,…,vₖ)$,~$v,…,v∈Γ∪X$,
% rather than~$γ(x₁,…,xₖ)$,~$x₁,…,xₖ∈X$ which it currently supports.
% In this extension, stack symbols are of pairs~$⟨ρ,γ(γ₁,…,γᵤ)⟩$
% where~$ρ∈Γ'$ is a rule as before, and~$γ(γ₁,…,γᵤ)$,~$γ∈Γᵤ$ and~$γ₁,…,γᵤ∈Γ$ is a
% \emph{promise} on the first level of the encoded tree.

% The tree encoding property is rephrased then to say that stack~$⟨ρ,p⟩α⊥$ is an
% encoding of a tree that acts on the promise~$p$ and is obtained by applying
% rewrite~$ρ$ to the tree encoded by~$⟨ρ,p⟩α⊥$. The promise stored at the top of
% the stack makes it possible to check while using bounded storage whether the
% left hand side of a pending rule~$ρ'$ matches the encoded tree. Also, the promise~$p$
% completely determines the promise after applying~$ρ'$.

The proof of~\cref{theorem:monadic} is completed with the following
emulation lemma.

\begin{lemma}\label{lemma:pda}
  For every run~$t₀,…,tᵢ$ of TPDA~$T$ that rewrites tree \[
    \begin{split}
      \qquad\qquad t₀ &=σₙ(σ_{n-1}(⋯(σᵢ(σ_{i-1}(⋯(σ₂(σ₁()))⋯)))⋯)) ⏎
      \intertext{\qquad into tree}
      \qquad\qquad tᵢ &=σₙ(σ_{n-1}(⋯(σᵢ(q(t)))⋯)),
    \end{split}
\] i.e., a tree representing the consumption of input letters~$σ₁…σ_{i-1}$
  being in state~$q∈Q$ with storage tree~$t∈Γ^▵$, there exists a run~$ι₀,…,ιᵢ$
  of PDA~$A$ which starts with instantaneous description \[
    \begin{split}
      \qquad\qquad ι₀=&⟨q₀,⊥,σ₁σ₂⋯σ_{i-1}σᵢ⋯σ_{n-1}σₙ⟩ ⏎
      \intertext{\qquad and ends with instantaneous description}
      \qquad\qquad ιᵢ=&⟨q,α,σᵢ⋯σ_{n-1}σₙ⟩,
    \end{split}
\] which represents~$A$ having consumed the same input letters as~$T$, being in
  the same state~$q$ as~$T$ and with stack~$α∈(Γ')^*$ which encodes tree~$t$
  of~$T$.
\end{lemma}

\begin{proof}
  Technical, by induction on~$i$.
\end{proof}

\subsection{Extension}\label{section:extension}
We propose that the conversion of restricted TPDA to PDA described
in~\cref{section:monadic} is applicable to the deterministic versions of the
automata, i.e., that for every restricted DTPDA there exists a DPDA which
accepts the same
language.

The PDA construction hinted in~\cref{section:monadic} has no distinctively
non-deterministic transitions, i.e., having the input restricted TPDA is
deterministic implies the composed PDA is also deterministic.

For every accumulating rewrite rule we assign a single transition
pushing its right-hand side onto the stack. Extracting rules, on the
other hand, may force us to iterate over the stack in an unbounded number
of~$𝜀$-transitions: We argue that this computation can be done
in a deterministic fashion, as in each of its steps is defined by a single
rewrite rule (on the stack's top) and a single child to be extracted.

The proof is by induction over the number of rewrite rules applied,~$n$.

\noindent\textbf{Inductive base:} We apply a single rewrite rule~$ρ$ to the bottom
term~$σ₁$.
The TPDA may consume~$σ₁$ if and only if~$ρ=σ₁→q(t)$,
for some state~$q$ and ground term~$t$. If such rule exists, then~$δ$ contains the
corresponding transition~$(q₀,σ,⊥,q,·→t)$, so~$A$ consumes~$σ$, moves to
state~$q$ and pushes~$·→t$ onto the stack, which now obviously encodes~$t$.
Otherwise, if such rule does not exist, then both automata get stuck.

\noindent\textbf{Inductive assumption:} We assume that~$T$
rewrites a subtree of its input into~$q(t)$ in~$n$ rewrite rule applications,
and that after~$A$ commits the corresponding transitions, its state is also~$q$
and its stack encodes~$t$.

\noindent\textbf{Inductive step:} We now show that if another rewrite by~$T$
yields~$q'(t')$, then after~$A$ commits the corresponding transitions its state
is also~$q'$, and its stack encodes~$t'$.

We assume the rewrite applied is consuming, i.e., that it is of the form~$
  ρ=σ(q(τ))→q'(τ'),$ involving a consumption of an input node, a change of state and a
manipulation of the storage. The proof for non-consuming rewrites, where
no input node is consumed, is very similar, and thus be omitted.





==> todo.tex <==
\thispagestyle{empty}
\newcommand{\zzzdone}{\rlap{$\square$}{\large\hspace{1pt}\checkmark}\hspace{-4pt}}%
\begin{itemize}[label=$\square$]
\item fix bib,
\item fix outline
\item[\zzzdone] organize in four items the long proof, no textual changes.
\item fix the list of symbols, 
\item[\zzzdone] revert to two stacks notation in abcdex1/x/yyy
\item format typelevelLR, Fling, Fluent
\end{itemize}
\begin{itemize}[label=$\square$]
\item 00: FSA fix acronym when expanded; I think FSA is readable but not TM or TA. Even ID is bad, but cannot help it. 
\item aa: disscuss type equaltity and subtyping similar to automata equality
\item capture: we may need to say that $aaa/asefs/$  is in the two stacks alphabet.
\item aa: introduce acronym for Yamazaki
\item aa: REVIVE FIG D.1
\item Automata: discuss complexity classes
\item Automata: explain bottom up must be trees.
\item Automata: explain empty stack monkey business
\item Automata: mention other crazy automata with aux storage
\item Do not forget to mention this in automata
\item ZZ: List of acronyms? words?
\item ZZ: List of grammar rules???
\end{itemize}

\eject
\pagenumbering{arabic}




==> toplas.tex <==
\subsection{Proof of \cref{lower:bound}}

We prove~$\|TA|⊆\|DPDA|$.
The proof is by construction: Given a tree automaton~$A$, we describe a DPDA~$A'$
that emulates~$A$.

\paragraph{States.}
Recall tree automaton~$A$ is stateless.
DPDA~$A'$ employs states~$Q'=❴q₀,q₁,…,qₘ❵$, where~$m$ is the maximal rank
of signatures in~$A$'s store alphabet~$Γ$.
Also, let~$q₀$ be the initial state of~$A'$, and the only accepting state,~$F'=❴q₀❵$.

\subsubsection{Intuition}
\label{section:intuition}

The challenge of the emulation is in using the DPDA's stack to encode the tree
store manipulated by the tree automaton.  To see that a plain prefix order
encoding of a tree in a stack does not work, consider applying the reducing
rewrite rule~$ρ₆=γ₂(x₁,x₂)→γ₃(x₂,γ₁(x₁),γ₀)$ to tree~$γ₂(t₁,t₂)$,~$t₁,t₂∈Γ^▵$.
In prefix order the stack is~$γ₂α₁α₂⊥$ where~$αᵢ$ is the stack encoding of
tree~$tᵢ$,~$i=1,2$. To emulate the rewrite a PDA moves to state~$q'$ and
pops~$γ₂$. But then, to maintain prefix encoding the remaining stack~$α₁α₂⊥$
should be rearranged to~$γ₃α₂γ₁α₁γ₀⊥$. Alas, the unbounded length of~$α₁$
and~$α₂$ makes this rearrangement impossible in the bounded memory available to
a PDA other than the stack itself.

A better encoding of the TPDA's tree by letting the PDA's stack employ rewrite
rules as its symbols: a tree~$t∈Γ^▵$ is encoded as a sequence of applications
of \emph{accumulating} rewrite rules stored in a stack, with the latest rewrite
at the stack's top. The earliest rewrite, stored at the stack's bottom is rule
of the form~$⊥→t$,~$t$ being a grounded term over~$Γ$, e.g., an encoding of the
leaf node~$γ₀$ is the sequence comprising the single rule~$ρ₀=⊥→γ₀$.
Also,~$ρ₃ρ₅ρ₀⊥$ is a stack encoding of~$t₅=γ₂(γ₂(γ₀,γ₀),γ₀)$, since applying
rule~$ρ₅$ to~$γ₀$, and then~$ρ₃$ yields~$t₅$. The encoding is not unique, e.g., \[
  \overbrace{ρ₃⋯ρ₃}ⁿρ₅γ₀⊥
\] is a stack encoding of~$t₅$ for all odd values of~$n$.

With this encoding, an application of any accumulating rewrite rule~$ρ$ to the
current tree is emulated by pushing~$ρ$ onto the stack. For example,
applying~$ρ₆$ and then~$ρ₄$ to tree~$t₅$ yields the
term~$γ₂(γ₂(γ₁(γ₀),t₂),t₂)$; to encode this term, rules~$ρ₆$ and~$ρ₄$ are
pushed onto the stack, as depicted in~\cref{figure:stack}.

\begin{figure}[H]
  \caption{Stack contents
    after applying rewrite rule~$ρ₅$, then~$n$ times~$ρ₃$ for some
    odd~$n$, then~$ρ₆$, and finally~$ρ₄$ to~$ρ₀=⊥→γ₀$.}
  \label{figure:stack}
  \adjustbox{max width=\textwidth}
  {\input{stack.tikz}}
\end{figure}

%To see that the encoding makes it is possible to match rules against the
%current tree in its encoded form, we assume for now that rewrite rules of the
%form~$γ(v₁,…,vₖ)→τ$ are restricted to the form~$γ(x₁,…,xₖ)→τ$, i.e., there are
%no rules such as~$γ₂(γ₃(⋯),x₁)→τ$ in which one alphabet symbol ($γ₃$) occurs as
%argument of another alphabet symbol~($γ₂$) in the left hand size of the rule.
%Later we will see how this assumption can be lifted.
%With this assumption and the presumed linearity of rules.

The PDA's finite control can use the stack's top to decide whether a certain
rule is applicable to the current tree. Rule~$ρ₄$ at the top of the stack in
the figure confirms that the current tree is of the form~$γ₂(t₁,t₂)$
with~$t₁,t₂∈Γ^▵$. Rules~$ρ₁$,~$ρ₂$,~$ρ₃$ and~$ρ₆$, indeed all rules whose left
hand is the term~$γ₂(x₁,x₂)$, match this tree. Regardless of the stack's top,
the current tree is matched by~$ρ₇$, and, more generally all rules of the
form~$x→τ$ whose left does not place any constraints on the matched tree.

As said, the encoding is preserved by always pushing accumulating rules.
Managing extracting rules is more tricky, requiring sometimes an unbounded
sequence of pop operations: Consider the application of extracting
rule \[
  ρ₂=γ₂(x₁,x₂)→x₂
\] to the stack depicted in \cref{figure:stack}. To
extract the \emph{second} child of the current tree we inspect rule~$ρ₄$ at the
top of the stack to infer that this second child is variable~$x₁$ of the
term~$γ₃(x₁,x₂,x₃)$ that matched the current tree prior to the application
of~$ρ₄$. Popping~$ρ₄$ obtains the stack encoding of the previous version of the
current tree. On this shorter stack, we need to find the first child
of~$γ₃(x₁,x₂,x₃)$. Popping rule~$ρ₆$, the problem is reduced to finding second
child of a tree~$γ₂(x₁,x₂)$. To encode the current tree after the rewrite~$ρ₂$
we need to further pop the~$n$ copies of~$ρ₃$ and then replace rule~$ρ₅$ at the
top of the remaining stack with rule~$γ₀→γ₂(γ₀,γ₀)$.

A similar replacement of the rule at the stack's top occurs when applying
rule~$ρ₁=γ₂(x₁,x₂)→x₁$ that extracts the first child of the tree encoded in the
figure. The right of~$ρ₄$, term~$γ₂(γ₂(x₂,x₁),x₁)$, specifies how this first
child depends on the tree before applying~$ρ₄$. Accumulating
rule~$ρ₄'=γ₃(x₁,x₂,x₃)→γ₂(x₂,x₁)$ then describes the combined application
of~$ρ₄$ and~$ρ₂$, and the encoding is preserved by replacing~$ρ₄$ by~$ρ₄'$ at
the top of the stack.

\subsubsection{Transition functions}
Having gained the intuition of the emulation, we now turn to providing the
technical details of the emulation behind the proof
of~\cref{theorem:monadic}.

Recall that PDA~$A$ uses the same alphabet as~$T$, and its set of states
is~$Q'=❴q₀❵∪Q∪Q×❴1,…,k❵$. The set~$Γ'$ of stack symbols of~$A$ comprises the
special bottom of stack symbol~$⊥$ and rules of the form~$τ→τ'$,
where~$τ∈❴⊥❵∪Γ⧋$ and~$τ'∈Γ⧋$.
It remains to describe~$δ$, the transition function of~$A$.

We say that an accumulating rewrite rule~$ρ'∈Γ'$ \emph{follows} another
accumulating rewrite rule~$ρ∈Γ'$ and write~$ρ⤳ρ'$, if~$ρ'$ is applicable after
applying~$ρ$. More exactly,~$ρ⤳ρ'$ if~$ρ'$ is a shallow match of every
tree encoded by a stack of the form~$ρα⊥$, for arbitrary~$α∈(Γ')^*$.

Considering the rules in \cref{figure:rules} we see that rule~$ρ₆$ which
assumes a tree whose root is~$γ₂$ follows~$ρ₃$,~$ρ₄$ and~$ρ₅$. Also, yields a
tree with root~$γ₃$, rule~$ρ₆$ is followed by~$ρ₄$ which requires~$γ₂$ root of
the input tree, and by rule~$ρ₇$ which is applicable to any tree.

%More
%generally, with the assumption an alphabet symbol cannot occur as an
%argument of another alphabet symbol in the left hand size of the rule, we can
%tell whether~$ρ⤳ρ'$ solely by comparing the root of the term in the right~$ρ$
%with the root of the term in the left of~$ρ'$.

More generally, with the restriction that at most one stack
node occurs in the left hand size of the rule, we can
tell whether~$ρ⤳ρ'$ solely by comparing the root of the term in the right~$ρ$
with the root of the term in the left of~$ρ'$.

For each rewrite rule present in~$R$, we construct transition(s) as follows.
Even with our simplifying assumption on the structure of standard rules,
There are quite a number of cases to consider:
\begin{description}
  \item[Standard Rules] By our transformation, these rules do not manipulate the tree storage.
        They come in two varieties:
        \begin{enumerate}
          \item~$σ(q(τ))→q'(τ)$, \emph{standard rule, inner node}: Introduce a
                transition~$(q,σ,ρ)→(q',ρ)$ for every stack symbol~$ρ$. These
                transition preserve the stack, consume letter~$σ$ and move to state~$q'$.
          \item~$σ→q(t)$, \emph{standard rule, leaf node}: Introduce stack
                symbol~$ρ=⊥→t$ and transition~${(q₀,σ,⊥)→(q,ρ⊥)}$. This transition
                initializes the stack with a rewrite that generates a non-empty tree~$t∈Γ^▵$
                from the stack's bottom.
        \end{enumerate}
  \item[Reduce Rules] Such a rule does not consider the input. It can be
        accumulating, and hence emulated by being pushing onto the stack,
        or extracting, and then emulated by a sequence of an unbounded number of
        stack pop operations, followed by a push of a new rule:
        \begin{enumerate}
          \item~$q(τ)→q'(τ')$, \emph{accumulating reduce rule}: Introduce stack
                symbol~$ρ'=τ→τ'$ and create transition~$(q,𝜀,ρ)→(q',ρ'ρ)$ for
                every~$ρ∈Γ'$ that satisfies~$ρ⤳ρ'$, i.e., push~$ρ'$, move
                to state~$q'$. This rule is applicable if the current state is~$q$
                and the stack's top, rewrite rule~$ρ$ is such that~$ρ'$ is
                applicable to the tree encoded in the stack.

          \item~$q(x)→q'(x)$, \emph{degenerate accumulating reduce rule}:
                Create transition~$(q,𝜀,ρ)→(q',ρ)$ for every~$ρ∈Γ'$. These
                transitions leaves the stack intact, but move from state~$q$ to
                state~$q'$.

          \item~$q(γ(x₁,…,xₖ,…,xᵤ))→q'(xₖ)$, \emph{extracting reduce rule},
                where~$u≤m$ is the rank of symbol~$γ$, and~$k$,~$1≤k≤u$, is the
                index of the extracted variable. Let the stack's top be
                rule~$ρ=τ→τ'$. We must then create transitions to extract~$τ'[k]$,
                the~$k$\xth child of~$τ'$, while preserving the stack encoding.

                \begin{enumerate}
                  \item If~$τ'[k]$ is a term which is not a variable, then as done
                        above in the application of~$ρ₁$ after~$ρ₄$, introduce a stack
                        symbol~$ρ'=τ→τ'[k]$. Rule~$ρ'$ is similar to~$ρ$, but rather
                        than rewriting the encoded tree to the full term~$τ'$, it
                        rewrites it to its subtree~$τ'[k]$. Rule~$ρ'$ is accumulating
                        by the assumption~$τ'[k]∉X$, and can therefore be used as a
                        symbol in the stack encoding of trees. To replace~$ρ$ by~$ρ'$
                        at the top of the stack, introduce
                        transition~$(q,𝜀,ρ)→(q',ρ')$. This transition also moves from
                        state~$q$ to state~$q'$.

                  \item Suppose that~$τ'[k]∈X$. Since~$ρ=τ→τ'$ is a
                        rule,~$\Vars(τ')⊆\Vars(τ)$, variable~$τ'[k]∈X$ must be present
                        in~$τ$. By the restrictions on monadic~$T$,~$τ$
                        is either a variable or a compound term of the form~$γ'(x₁,…,x_{u'})$.

                        If~$τ$ is also a variable, then it must be the variable~$τ'[k]$,
                        so~$τ'[k]$ is precisely the tree encoded by the stack prior to
                        the application of~$ρ$. Introduce then
                        transition~${(q,𝜀,ρ)→(q',𝜀)}$, which pops~$ρ$ from the stack
                        and moves to~$q'$.

                        Otherwise,~$τ'[k]$ is variable~$xᵢ$ appearing in~$τ=γ'(x₁,…,x_{u'})$.
                        Automaton~$A$ must proceed to extract the~$i$\xth child of the
                        tree prior to the rewrite~$ρ$. Introduce then
                        transition~${(q,𝜀,ρ)→(⟨q',i⟩,ρ)}$, which leaves the stack
                        intact, but moves to intermediate state~$⟨q',i⟩$. Being in
                        state~$⟨q',i⟩$ tells~$A$ to ‟\emph{extract child~$i$ of the
                          currently encoded tree and then move to state~$q'$}”.
                \end{enumerate} % inner
        \end{enumerate} % outer
\end{description}

We still need to add transitions to realize the intent of the above mentioned
intermediate states. For intermediate state~$⟨q,k⟩$ and rule~$ρ=τ→τ'$, where
the rank of the symbol in the root of~$τ'$ is no less than~$k$, let~$τ'[k]$ be
the~$k$\xth child of~$τ'$, and,
\begin{itemize}
  \item if~$τ'[k]∉X$, introduce accumulating rule~$p'=τ→τ'[k]$ as stack symbol, and
        transition~$(⟨q,k⟩,𝜀,ρ)→(q,ρ')$ to move to destination state~$q$ and
        replace a top of stack~$ρ$ with~$ρ'$ whenever in state~$⟨q,k⟩$ and top
        of stack is~$ρ$;
  \item if~$τ'[k]$ is a variable~$x$ then~$τ=x$. Introduce then
        transition~$(⟨q,k⟩,𝜀,ρ)→(q,𝜀)$ to pop~$ρ$ and move to destination state~$q$.
  \item otherwise,~$τ'[k]$ is some variable~$xᵢ$;
        then introduce transition~$(⟨q,k⟩,𝜀,ρ)→(⟨q,i⟩,𝜀)$ to pop~$ρ$ and
        proceed the search down the stack for the~$i$\xth child of the tree encoded
        by the remaining stack, and then move to state~$q$.
\end{itemize}

We therefore have that accumulating rules of~$R$ are emulated by precisely one
transition from state~$q$,~$q∈❴q₀❵∪Q$ to state~$q'∈Q$. Extracting rules
of~$T$ are emulated by an unbounded number of transitions, starting in~$q∈Q$,
possibly going through some intermediate states of the form~$⟨q',·⟩$, each
popping a rule of the stack, and ending in a state~$q'∈Q$ and a push of a rule.

Review the definition of~$δ$ to better understand the set~$Γ'$: A standard
rule in~$R$ that operates on a leaf node introduced a symbol of the form~$⊥→t$.
A reduce rule in~$R$ could be accumulating, in which case it introduces a
single element to~$Γ'$. However if this rule is extracting,
it can introduce many. Observe however that a rule~$p'$ is introduced only if
there exists a rule~$ρ∈Γ'$ such that~$ρ=τ→τ'$ and~$ρ'=τ→τ'[k]$. Since the
description of~$ρ'$ is shorter than the description of~$ρ'$, set~$Γ'$ must be
finite.

% Although not strictly necessary for the proof of \cref{theorem:monadic}, we
% explain now how the emulation is extended to handle rules such
% as~$γ₂(γ₃(⋯),x₁)→τ$: To make this happen, we need to extend the~$⤳$ relation
% so that it supports matches of patterns~$γ(v₁,…,vₖ)$,~$v,…,v∈Γ∪X$,
% rather than~$γ(x₁,…,xₖ)$,~$x₁,…,xₖ∈X$ which it currently supports.
% In this extension, stack symbols are of pairs~$⟨ρ,γ(γ₁,…,γᵤ)⟩$
% where~$ρ∈Γ'$ is a rule as before, and~$γ(γ₁,…,γᵤ)$,~$γ∈Γᵤ$ and~$γ₁,…,γᵤ∈Γ$ is a
% \emph{promise} on the first level of the encoded tree.

% The tree encoding property is rephrased then to say that stack~$⟨ρ,p⟩α⊥$ is an
% encoding of a tree that acts on the promise~$p$ and is obtained by applying
% rewrite~$ρ$ to the tree encoded by~$⟨ρ,p⟩α⊥$. The promise stored at the top of
% the stack makes it possible to check while using bounded storage whether the
% left hand side of a pending rule~$ρ'$ matches the encoded tree. Also, the promise~$p$
% completely determines the promise after applying~$ρ'$.

The proof of~\cref{theorem:monadic} is completed with the following
emulation lemma.

\begin{lemma}\label{lemma:pda}
  For every run~$t₀,…,tᵢ$ of TPDA~$T$ that rewrites tree \[
    \begin{split}
      \qquad\qquad t₀ &=σₙ(σ_{n-1}(⋯(σᵢ(σ_{i-1}(⋯(σ₂(σ₁()))⋯)))⋯)) ⏎
      \intertext{\qquad into tree}
      \qquad\qquad tᵢ &=σₙ(σ_{n-1}(⋯(σᵢ(q(t)))⋯)),
    \end{split}
\] i.e., a tree representing the consumption of input letters~$σ₁…σ_{i-1}$
  being in state~$q∈Q$ with storage tree~$t∈Γ^▵$, there exists a run~$ι₀,…,ιᵢ$
  of PDA~$A$ which starts with instantaneous description \[
    \begin{split}
      \qquad\qquad ι₀=&⟨q₀,⊥,σ₁σ₂⋯σ_{i-1}σᵢ⋯σ_{n-1}σₙ⟩ ⏎
      \intertext{\qquad and ends with instantaneous description}
      \qquad\qquad ιᵢ=&⟨q,α,σᵢ⋯σ_{n-1}σₙ⟩,
    \end{split}
\] which represents~$A$ having consumed the same input letters as~$T$, being in
  the same state~$q$ as~$T$ and with stack~$α∈(Γ')^*$ which encodes tree~$t$
  of~$T$.
\end{lemma}

\begin{proof}
  Technical, by induction on~$i$.
\end{proof}

